A Simple Framework for Secure Key Leasing

Secure key leasing (a.k.a. key-revocable cryptography) enables us to lease a cryptographic key as a quantum state in such a way that the key can be later revoked in a verifiable manner. We propose a simple framework for constructing cryptographic primitives with secure key leasing via the certified deletion property of BB84 states. Based on our framework, we obtain the following schemes. - A public key encryption scheme with secure key leasing that has classical revocation based on any IND-CPA secure public key encryption scheme. Prior works rely on either quantum revocation or stronger assumptions such as the quantum hardness of the learning with errors (LWE) problem. - A pseudorandom function with secure key leasing that has classical revocation based on one-way functions. Prior works rely on stronger assumptions such as the quantum hardness of the LWE problem. - A digital signature scheme with secure key leasing that has classical revocation based on the quantum hardness of the short integer solution (SIS) problem. Our construction has static signing keys, i.e., the state of a signing key almost does not change before and after signing. Prior constructions either rely on non-static signing keys or indistinguishability obfuscation to achieve a stronger goal of copy-protection. In addition, all of our schemes remain secure even if a verification key for revocation is leaked after the adversary submits a valid certificate of deletion. To our knowledge, all prior constructions are totally broken in this setting. Moreover, in our view, our security proofs are much simpler than those for existing schemes.

==> OW-to-IND.tex <==
% !TEX root = main.tex




\section{OW-KLA to IND-KLA Transformation for PKE-SKL}\label{sec:OW-to-IND-classicalcert} 
\subsection{Preparation}
We need the quantum Goldreich-Levin lemma established by \cite{C:CLLZ21} based on \cite{AC02}.
\begin{lemma}[Quantum Goldreich-Levin with Quantum Auxiliary Input~{\cite[Lemma~B.12]{C:CLLZ21}}]\label{lem:QGL}
There exists a QPT algorithm $\qExt$ that satisfies the following.
Let $n \in \mathbb{N}$, $x\in \bit^n$, $\epsilon\in [0,1/2]$,  and $\qA$ be a quantum algorithm with a quantum auxiliary input $\qaux$ such that    
\begin{align}
    \Pr\left[\qA(\qaux,r)\ra x\cdot r ~\middle |~ r\gets \bit^n\right]
    \geq \frac{1}{2}+\epsilon.
\end{align}
%\begin{align}
%    \left|
%    \Pr\left[\qA(\qaux,r,(x\cdot r \mod 2) )\ra 1 \right]
%    -
%    \Pr\left[\qA(\qaux,r,u)\ra 1 \right]
%    \right|
%    \geq \epsilon
%\end{align}
%where $r\gets \bit^n$ and $u\gets \bit$.
%Then there exists a quantum algorithm $\qExt$ (that does not depend on $x$) 
%such that
Then, we have
\begin{align}
    \Pr\left[\qExt([\qA],\qaux)\rightarrow x \right]\geq 4\epsilon^2.
\end{align}
where $[\qA]$ means the description of $\qA$. %\takashi{The description of $\qA$ is classical. Should we use a different notation?}\shweta{Yes, I would say so.}\takashi{How about the above notation $[\qA]$?} \shweta{Looks fine.}
%Moreover, there is an efficient procedure to construct $\qExt$ from the description of $\qA$.
%Moreover, the running-time of $\qExt$ is $2T_{\qA} + O(\ell)$. 
%\takashi{By running-time, I mean the number of gates.}
\end{lemma}




\subsection{Transformation}
\begin{lemma}[Restatement of \Cref{lem:ow-ind}]\label{lem:ow-ind_app}
If there exists a OW-VRA secure PKE-SKL scheme with classical verification, then there exists an IND-VRA secure PKE-SKL scheme with classical verification.
\end{lemma}
\begin{proof}  
We remark that the proof is very similar to that of... 
Let $\OWSKL=(\OWSKL.\qKG, \OWSKL.\Enc, \OWSKL.\qDec,\OWSKL.\qDel,\OWSKL.\Vrfy)$ be a OW-VRA secure PKE-SKL scheme with classical verification whose message space is $\bit^n$. Then, we construct an IND-VRA secure PKE-SKL scheme with classical verification $\INDSKL=(\INDSKL.\qKG, \INDSKL.\Enc, \INDSKL.\qDec,\INDSKL.\qDel,\INDSKL.\Vrfy)$ whose message space is $\bit$ as follows. 
\begin{description}
\item[$\INDSKL.\qKG(1^\secp)\ra(\ek,\qdk,\vk)$:] On input the security parameter $1^\lambda$, 
run $(\ek,\qdk,\vk)\gets \OWSKL.\qKG(1^\secp)$ and output $(\ek,\qdk,\vk)$.

\item[$\INDSKL.\Enc(\ek,\msg)\ra\INDSKL.\ct$:]On input an encryption key $\ek$ and a message $\msg \in \bit$, 
choose $r,x\gets \bit^n$, 
generate $\OWSKL.\ct\gets \OWSKL.\Enc(\ek,x)$, 
set $b \seteq (x\cdot r)\oplus \msg$,
and output a ciphertext $\INDSKL.\ct\seteq (\OWSKL.\ct,r,b)$.

\item[$\INDSKL.\qDec(\qdk,\INDSKL.\ct)\ra\tilde{\msg}$:] On input a decryption key $\qdk$ and a ciphertext $\INDSKL.\ct= (\OWSKL.\ct,r,b)$, 
compute $\tilde{x}\gets \OWSKL.\qDec(\qdk,\OWSKL.\ct)$
and output $\tilde{\msg}\seteq (\tilde{x}\cdot r)\oplus b$.

\item[$\INDSKL.\qDel(\qdk)$:] On input a decryption key $\qdk$, output $\cert\gets\OWSKL.\qDel(\qdk)$.

\item[$\INDSKL.\qVrfy(\vk,\cert)\ra\top/\bot$:] On input a verification key $\vk$ and a (possibly malformed) cert $\cert$, run $\OWSKL.\Vrfy(\vk,\cert)$ and
output whatever $\OWSKL.\Vrfy$ outputs.  
\end{description}
The decryption correctness and verification correctness of $\INDSKL$ immediately follow from those of $\OWSKL$. 
In the following, we prove that $\INDSKL$ is IND-VRA secure assuming that $\OWSKL$ is OW-VRA secure. 
Toward contradiction, suppose that $\INDSKL$ is not IND-VRA secure. Then, there is a QPT adversary $\qA$ such that $\advb{\INDSKL,\qA}{ind}{vra}(\secp)$ is non-negligible. Without loss of generality, we assume that 
\begin{align} \label{eq:IND_A_wins}
\Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{vra} (1^\secp,\coin) \ra \coin]\ge 1/2+\epsilon(\secp)
\end{align}
for a non-negligible $\epsilon(\secp)$.  Without loss of generality, we may assume $\epsilon(\secp)>0$ for all $\secp\in \mathbb{N}$. 
%Let $S\seteq \{\secp\in \mathbb{N}:\epsilon(\secp)>0\}$. Then $S$ is an infinite set. Below, we focus on security parameters $\secp$ that belong $S$.  
Since $\INDSKL$ is a bit encryption, we assume that the challenge message pair $(\msg_0,\msg_1)$ is $(0,1)$ without loss of generality.  
We divide $\qA$ into the following two stages $\qA_0$ and $\qA_1$: 
\begin{description}
\item[$\qA_0(\ek,\qdk)\rightarrow (\cert,\qst_\qA)$:] Upon receiving $(\ek,\qdk)$ from the challenger, output a classical certificate $\cert$ and a quantum state $\qst_\qA$. 
\item[$\qA_1(\qst_\qA,\vk,\INDSKL.\ct)\rightarrow \coin'$:] Upon receiving the state $\qst_\A$ from $\qA_0$, and $\vk$ and $\INDSKL.\ct=(\OWSKL.\ct,r,b)$ from the challenger, output $\coin'$.  
\end{description} 

We have 
\begin{align}
&\Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{vra} (1^\secp,\coin) \ra \coin]\\
&=\Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{vra} (1^\secp,\coin) \ra \coin \wedge \Vrfy(\vk,\cert)=\top]\\
&+\Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{vra} (1^\secp,\coin) \ra \coin \wedge \Vrfy(\vk,\cert)=\bot]\\
&=
\Pr[\Vrfy(\vk,\cert)=\returned]
\cdot \Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{vra} (1^\secp,\coin) \ra \coin \mid \Vrfy(\vk,\cert)=\returned]\\
&+\frac{1}{2}(1-\Pr[\Vrfy(\vk,\cert)=\returned]). \label{eq:advantage_A_decompose}
\end{align}
%By \cref{eq:IND_A_wins,eq:advantage_A_decompose} and $\Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{kla} (1^\secp,\coin) \ra \coin \mid V=\returned]\le 1$, we have 
%\begin{align}\label{eq:returned_prob}
% \Pr[V=\returned]\ge 2\epsilon(\secp).     
%\end{align}
By \cref{eq:IND_A_wins,eq:advantage_A_decompose}, 
we have%\footnote{For $\secp$ such that$\epsilon(\secp)=\Pr[\Vrfy(\vk,\cert)=\returned]=0$, we treat $\frac{\epsilon(\secp)}{\Pr[\Vrfy(\vk,\cert)=\returned]}=0$. }   
\begin{align}\label{eq:conditioned_on_returned_prob}
 \Pr_{\coin\gets \bit}[\expb{\INDSKL,\qA}{ind}{kla} (1^\secp,\coin) \ra \coin \mid \Vrfy(\vk,\cert)=\returned]\ge \frac{1}{2}+\frac{\epsilon(\secp)}{\Pr[\Vrfy(\vk,\cert)=\returned]}.
\end{align}

Then, we construct an adversary $\qB=(\qB_0,\qB_1)$ against OW-KLA security of $\OWSKL$ that works as follows. 
\begin{description}
\item[$\qB_0(\ek,\qdk)\rightarrow (\cert,\qst_\qA)$:]  
This is identical to $\qA_0$. Specifically, run $(\cert,\qst_\qA)\gets \qA_0(\ek,\qdk)$ and output $\cert$ and $\qst_\qA$.
%Upon receiving $(\ek,\qdk)$ from $\qC$, run $\qst_\qA\gets \A_0^{\Oracle{\qVrfy}}(\ek,\qdk)$  and send $\widetilde{\qdk}$ to $\qC$ while keeping $\qst_\qA\seteq(\ek,\qst_\qA)$ as its internal state. 
\item[$\qB_1(\qst_\qA,\vk,\OWSKL.\ct)\rightarrow x$:] Upon receiving $\qst_\qA$ from $\qB_0$, and $\vk$ and $\OWSKL.\ct$ from the challenger, set $\qaux\seteq (\qst_\qA,\vk,\OWSKL.\ct)$ and define an algorithm $\qA'$ as follows.
\begin{description}
\item[$\qA'(\qaux,r)$:]
On input $\qaux=(\qst_\qA,\vk,\OWSKL.\ct)$ and $r\in \bit^n$,  choose $b\gets \bit$, 
set $\INDSKL.\ct=(\OWSKL.\ct,r,b)$,  
run $\coin' \gets \qA_1(\qst_\qA,\vk,\INDSKL.\ct)$, and output $\coin'\oplus b$.  
\end{description}
Run $x\gets \qExt([\qA'],\qaux)$, and output $x$ where 
$\qExt$ is the algorithm as in \Cref{lem:QGL} and
$[\qA']$ is the description of $\qA'$.
\end{description}

In the following, we show that $\qB$ breaks OW-KLA security of $\OWSKL$. 
Let $\qG$ be an algorithm that works as follows.
\begin{description}
\item[$\qG(1^\secp)$:] 
Generate $(\ek,\qdk,\vk)\gets\OWSKL.\qKG(1^\secp)$, 
$(\cert,\qst_\qA)\gets \A_0(\ek,\qdk)$,   
%and let $\qst'_\qA$ be $\A$'s internal state after the execution of $\qVrfy$., \footnote{Since $\widetilde{\qdk}$ and $\qst_\qA$ may be entangled, the stare may change by $\qVrfy$.}   
$x\gets \bit^n$, and 
$\OWSKL.\ct\gets \OWSKL.\Enc(\ek,x)$.
Let $V\seteq \returned$ if $\Vrfy(\vk,\cert)=\returned$ and $V\seteq \unreturned$ otherwise.    
Output $(V,\qst_\qA,\vk,\OWSKL.\ct,x)$. 
\end{description}
%By \Cref{eq:returned_prob}, we have 
%\begin{align}
%    \Pr_{(V,\qst_\qA,\OWSKL.\ct,x)\gets \qG(1^\secp)}[V=\returned]\ge 2\epsilon(\secp). 
%\end{align}

By \cref{eq:conditioned_on_returned_prob} and a standard averaging argument,  
for at least $\frac{\epsilon(\secp)}{2\Pr[V=\returned]}$-fraction of $(V,\qst_\qA,\vk,\OWSKL.\ct,x)$ generated by $\qG(1^\secp)$ conditioned on $V=\returned$, we have 
\begin{align} 
    \Pr\left[
    \A_1(\qst_\qA,\vk,\INDSKL.\ct)\rightarrow \coin
    \right]\ge \frac{1}{2}+\frac{\epsilon(\secp)}{2\Pr[V=\returned]}\ge \frac{1}{2}+\frac{\epsilon(\secp)}{2}
\end{align}
where $\coin\gets \bit$, 
    $r\gets \bit^n$,  
    $b\seteq (x\cdot r)\oplus \coin$, and  
    $\INDSKL.\ct= (\OWSKL.\ct,r,b).$
    
Therefore, for at least $\frac{\epsilon(\secp)}{2}$-fraction of $(V,\qst_\qA,\vk,\OWSKL.\ct,x)$ generated by $\qG(1^\secp)$, we have 
\begin{align}\label{eq:IND_A_wins_rewrite_again} 
    \Pr\left[
    \A_1(\qst_\qA,\vk,\INDSKL.\ct)\rightarrow \coin
    \right]\ge \frac{1}{2}+\frac{\epsilon(\secp)}{2}
\end{align}
where $\coin\gets \bit$, 
    $r\gets \bit^n$,  
    $b\seteq (x\cdot r)\oplus \coin$, and  
    $\INDSKL.\ct= (\OWSKL.\ct,r,b).$

%for all $\secp \in S$.
For such $(V,\qst_\qA,\vk,\OWSKL.\ct,x)$, if we let $\qaux=(\qst_\qA,\vk,\OWSKL.\ct)$, \cref{eq:IND_A_wins_rewrite_again} directly implies  
\begin{align}
\Pr_{r\gets \bit^n}\left[\qA'(\qaux,r)\ra x\cdot r\right]\geq \frac{1}{2}+\frac{\epsilon(\secp)}{2}.
\end{align}
Therefore, by \Cref{lem:QGL}, we have 
\begin{align} \label{eq:ext_succeed}
    \Pr\left[\qExt([\qA'],\qaux)\rightarrow x \right]\geq \epsilon(\secp)^2.
\end{align}
Since \cref{eq:ext_succeed} \emph{and} $V=\returned$ hold at the same time for at least $\frac{\epsilon(\secp)}{2}$-fraction of $(V,\qst_\qA,\vk,\OWSKL.\ct,x)$, we have  
\begin{align}
    \Pr_{ (V,\qst_\qA,\vk,\OWSKL.\ct,x)\gets \qG(1^\secp) }\left[
    V=\returned
    \wedge
    \qB_1(\qst_\qA,\vk,\OWSKL.\ct)\rightarrow x 
    \right]\ge \frac{\epsilon(\secp)^3}{2}.
\end{align} 
By the definitions of $\qB=(\qB_0,\qB_1)$ and $\qG$ and the assumption that $\epsilon(\secp)$ is non-negligible, this implies that $\qB$ breaks OW-KLA security of $\OWSKL$. 
\end{proof}






==> PRFSKL-from-TPRF.tex <==
% !TEX root = main.tex

\newcommand{\AccVrfy}{\mathtt{AccVrfy}}
\newcommand{\Samplerev}{\overline{\Sample}}
\newcommand{\VKG}{\algo{VKG}}
\newcommand{\tlpsi}{\widetilde{\psi}}

\section{Construction of PRF-SKL with Classical Certificate}\label{sec:PRFSKL}
\takashi{This construction will not be included in the final version since we found a simpler construction.}


\fuyuki{I tried to write down the construction directly, but It was too complicated. Thus, it is better to introcude something like the following primitive as an intermediate primitive. The formalization of it is tentative. We might want to consider an intermediate primitive to achieve signature with secure key leasing.}

\subsection{Tailored Pseudorandom Function for BB84 State}\label{TPRFBB84}

\begin{definition}[Tailored PRF for BB84 state]
A tailored PRF for BB84 state $\TPRF$ with the domain $\Domprf$ and the range $\Ranprf$ is a tuple of six algorithms $(\KG, \qQKG,\Eval, \qQEval,\qDel,\Vrfy)$. 
\begin{description}
%\item[$\Setup(1^\secp,1^{\numkey})\ra\msk$:] The setup algorithm takes a security parameter $1^\lambda$ and a collusion bound $1^{\numkey}$, and outputs a master secret key $\msk$.
\item[$\KG(1^\secp,1^n)\ra\msk$:] The key generation algorithm takes a security parameter $1^\lambda$ and a BB84 parameter $n$, and outputs a master secret key $\msk$.

\item[$\qQKG(\msk,\ket{\psi_1}\tensor\cdots\tensor\ket{\psi_n})\ra\qsk$:] The quantum key generation algorithm takes a master secret key $\msk$ and a $n$-qubit quantum state $\ket{\psi_1}\tensor\cdots\tensor\ket{\psi_n}$, and outputs a quantum secret key $\qsk$.

\item[$\VKG(\msk,(x_i)_{i\in[n]:\theta[i]=1},\theta)\ra\vk$:] The verification key generation algorithm takes a master secret key $\msk$, substring $(x_i)_{i\in[n]:\theta[i]=1}$ of $x$, and $\theta$, and outputs a verification key $\vk$.

\item[$\Eval(\msk,\prfinp)\ra \prfout$:] The evaluation algorithm takes a master secret key $\msk$ and an input $\prfinp \in \Domprf$, and outputs a value $\prfout$.

\item[$\qQEval(\qsk,\prfinp)\ra \prfout$:] The quantum evaluation algorithm takes a quantum secret key $\qsk$ and an input $\prfinp \in \Domprf$, and outputs a value $\prfout$.

\item[$\qDel(\qsk)\ra\cert$:] The deletion algorithm takes a secret key $\qsk$, and outputs a classical string $\cert$.

\item[$\Vrfy(\vk,\cert)\ra\top/\bot$:] The verification algorithm takes a verification key $\vk$ and a deletion certificate $\cert$, and outputs $\top$ or $\bot$. This algorithm is deterministic.


\item[Evaluation correctness:]For every $\prfinp \in \Domprf$ and $x,\theta\in\bit^n$, we have
\begin{align}
\Pr\left[
\qQEval(\qsk, \prfinp) \allowbreak = \Eval(\msk,\prfinp)
\ \middle |
\begin{array}{ll}
\msk\gets\KG(1^\secp,1^n)\\
\qsk\gets\qQKG(\msk,\ket{x_\theta})
\end{array}
\right] 
=1-\negl(\secp).
\end{align}

\item[Verification correctness:]For every $x,\theta\in\bit^n$, we have 
\begin{align}
\Pr\left[
\Vrfy(\vk,\cert)=\top
\ \middle |
\begin{array}{ll}
\msk\gets\KG(1^\secp,1^n)\\
\qsk\gets\qQKG(\msk,\ket{x_\theta})\\
\vk\gets\VKG(\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta)\\
\cert\gets\qDel(\qsk)
\end{array}
\right] 
=1-\negl(\secp).
\end{align}
\end{description}
\end{definition}

\begin{definition}[Extractability on Hadamard Basis Position:]\label{def:ext-had-basis-pos}
%Let $\TPRF=(\KG,\qQKG,\Eval,\qQEval,\qDel,\Vrfy)$ be a tailored PRF scheme for BB84 state.
We say that $\TPRF$ satisfies extractability on Hadamard basis position if there exists a deterministic polynomial time algorithm $\Ext$ such that for every $x,\theta\in\bit^n$, $\msk\gets\KG(1^\secp,1^n)$, $\vk\gets\VKG(\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta)$, and a string $\cert$, if $\Vrfy(\vk,\cert)=\top$ holds, then we have $\Ext(\msk,\theta,\cert)=(x[i])_{i\in[n]:\theta[i]=1}$. 
\end{definition}




We next define simulatability on computational basis position.
Before defining it, we define the the distributions $D$ and $\Drev$.
\begin{description}
\item[$D$:]Generate $\beta\gets\bit$, $\prfinp\gets\Domprf$, $\prfout_0\gets\Eval(\msk,\prfinp)$, and $\prfout_1\gets\Ranprf$. Output $(\beta,\prfinp,\prfout_\beta)$.
\item[$\Drev$:]Generate $(\beta,\prfinp,\prfout)\gets D$. Output $(1\oplus \beta,\prfinp,\prfout)$.
\end{description}
Namely, $D$ is the distribution that outputs a PRF evaluation if the first bit $\beta=0$ and a random value if the first bit $\beta=1$, and $\Drev$ is its opposite (i.e., a PRF evaluation if $\beta=1$ and a random value if $\beta=0$).
We define simulatability on computational basis position that guarantees that there exists a simulator such that an adversary given $\qsk$ cannot distinguish an output of $\Sim$ with the input $\msk$ and $i\in[n]$ from an output of $D$ if $x[i]=0$ and from that of $\Drev$ if $x[i]=1$.


\begin{definition}[Simulatability on Computational Basis Position]\label{def:sim-comp-bisis-pos}
%Let $\TPRF=(\KG,\qQKG,\Eval,\qQEval,\qDel,\Vrfy)$ be a tailored PRF scheme for BB84 state.
Let $\Sim$ be a QPT simulation algorithm.
We define the experiment $\expt{\qA,\TPRF,\Sim}{sim\textrm{-}cbp}(\secp,\coin)$ as follows.
\begin{enumerate}
\item $\qA$ sends $(x,\theta,i^*)$ satisfying $\theta[i^*]=0$ to the challenger. The challenger generates $\msk \gets \KG(1^\secp,1^n)$, $\qsk\gets\qQKG(\msk,\ket{x_\theta})$, and $\vk\gets\VKG(\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta)$, and sends $\qsk$ and $\vk$ to $\qA$.
\item $\qA$ can get access to the following oracle.
\begin{description}
%\item[$\Oracle{vrfy}$:] On input $\cert$, it returns $\Vrfy(x,\theta,\msk,\cert)$.
\item[$\Oracle{sim}$:] On input $j\in[n]$, it returns $\Sim(\msk,j)$.
%\item[$\Oracle{eval}$:]It generates $x\gets\Domprf$ and returns $(x,\Eval(\prfk,x))$.\fuyuki{To Do: remove.}
%\item[$\Oracle{ext}$:]On input $(x,y)$, it computes $\prfk^\prime \gets\KeyExtract(\xk,(x,y))$.
%If $\prfk'=\prfk$, it returns special symbol $\challenge$. Otherwise, it returns $\prfk'$.
\end{description}

\item Let $\Dreal{i^\ast}$ be the following distribution. Note that $\Dreal{i^\ast}$ is identical with $D$ if $x[i^\ast]=0$ and with $\Drev$ if $x[i^\ast]=1$.
\begin{description}
\item[$\Dreal{i^\ast}$:]Generate $\beta\gets\bit$ and $\prfinp\gets\Domprf$. Then, if $\beta=x[i^\ast]$, generate $\prfout\gets\Eval(\msk,\prfinp)$, and otherwise, compute $\prfout\gets\Ranprf$. Output $(\beta,\prfinp,\prfout)$.
\end{description}
If $\coin=0$, the challenger samples $(\beta,\prfinp,\prfout)\gets\Dreal{i^\ast}$.
If $\coin=1$, the challenger generates $(\beta,\prfinp,\prfout)\gets\Sim(\msk,i^\ast)$.
The challenger sends $(\beta,\prfinp,\prfout)$ to $\qA$.


\item When $\qA$ terminates with output $\coin^\prime$, the challenger outputs $1$ if $\coin=\coin^\prime$ and $0$ otherwise.
\end{enumerate}

We say that $\TPRF$ satisfies simulatability on computational basis position if there exists QPT $\Sim$ such that for every QPT $\qA$, we have
\begin{align}
\adva{\qA,\TPRF,\Sim}{sim\textrm{-}cbp}(\secp)=
\abs{
\Pr[\expt{\qA,\TPRF,\Sim}{sim\textrm{-}cbp}(\secp,0)=1]
-\Pr[\expt{\qA,\TPRF,\Sim}{sim\textrm{-}cbp}(\secp,1)=1]
} =\negl(\secp).
\end{align}
\end{definition}

\begin{definition}[Quantum Simulatability on Computational Basis Position]\label{def:qsim-comp-bisis-pos}
We define the experiment $\expc{\qA,\TPRF,\Sim}{q}{sim}{cbp}(\secp,\coin)$ in the same way as $\expb{\qA,\TPRF,\Sim}{sim}{cbp}(\secp,\coin)$ except that $\qA$ can get access to the following oracle instead of $\Oracle{sim}$ in the step 2.
\begin{description}
\item[$\Oracle{qsim}$:]Given $j\in[n]$ and two registers $\qreg{R}$ and $\qreg{T}$, it applies the map $\ket{r}_{\qreg{R}}\ket{t}_{\qreg{T}}\ra\ket{r}_{\qreg{R}}\ket{t\oplus\Sim(\msk,j;r)}_{\qreg{T}}$ to $\qreg{R}$ and $\qreg{T}$ and returns the registers.
\end{description}
We say that $\TPRF$ satisfies quantum simulatability on computational basis position if there exists QPT $\Sim$ such that for every QPT $\qA$, we have
\begin{align}
\advc{\qA,\TPRF,\Sim}{q}{sim}{cbp}(\secp)=
\abs{
\Pr[\expc{\qA,\TPRF,\Sim}{q}{sim}{cbp}(\secp,0)=1]
-\Pr[\expc{\qA,\TPRF,\Sim}{q}{sim}{cbp}(\secp,1)=1]} =\negl(\secp).
\end{align}
\end{definition}


\subsection{PRF-SKL from Tailored PRF for BB84 State}
\fuyuki{I think we can extend our PKR-SKL into constrained PRF with secure key leasing.}
\takashi{May extend to constrained-hiding constrained PRFs as well? Then that will also give single-key succinct functional encryption (i.e., resubale garbled circuits) with SKL by using the construciton of Canneti-Chen \url{https://eprint.iacr.org/2017/143.pdf}. But that might be also possible by using GKPVZ as well \url{https://eprint.iacr.org/2012/733.pdf}.}\takashi{I found it's tricky how we should define CPRF-SKL. If we define it in a naive way, it probably follows from a simple XOR of PRF-SKL and plain CPRF.}
We construct a PRF-SKL scheme with classical certificate $\PRFSKL=(\PRFSKL.\qKG,\PRFSKL.\Eval, \PRFSKL.\qLEval,\allowbreak\PRFSKL.\qDel,\PRFSKL.\Vrfy)$ from Tailored PRF scheme for BB84 state $\TPRF=(\TPRF.\KG,\TPRF.\qQKG, \TPRF.\Eval,\allowbreak \TPRF.\qQEval,\TPRF.\qDel,\TPRF.\Vrfy)$.\mor{TPRF.VKG nuketeru}


\begin{description}
\item[$\PRFSKL.\qKG(1^\secp)$:] $ $
\begin{itemize}
    \item Generate $x,\theta\gets\bit^n$.
    \item Generate $\TPRF.\msk\gets\TPRF.\KG(1^\secp,1^{n+1})$.
    \item Generate $\TPRF.\qsk\gets\TPRF.\qQKG(\TPRF.\msk,\ket{x_\theta}\tensor\ket{0})$.
    \item Generate $\TPRF.\vk\gets\TPRF.\VKG(\TPRF.\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta\|0)$.
    \item Output $\msk\seteq\TPRF.\msk$, $\qsk\seteq\TPRF.\qsk$, and $\vk\seteq\TPRF.\vk$.
\end{itemize}


\item[$\PRFSKL.\Eval(\msk,\prfinp)$:] $ $
\begin{itemize}
    \item Parse $\msk= \TPRF.\msk$.
    \item Output $\prfout\gets\TPRF.\Eval(\TPRF.\msk,\prfinp)$. 
\end{itemize}
 
\item[$\PRFSKL.\qLEval(\qsk,\prfinp)$:] $ $
\begin{itemize}
   \item Parse  $\qsk= \TPRF.\qsk$.
   \item Output $\prfout\gets\TPRF.\qQEval(\TPRF.\qsk,\prfinp)$.
\end{itemize}

\item[$\PRFSKL.\qDel(\qsk)$:] $ $
\begin{itemize}
\item Parse $\qsk= \TPRF.\qsk$.
\item Output $\cert\gets\TPRF.\qDel(\TPRF.\qsk)$.
\end{itemize}


\item[$\TPRF.\Vrfy(\vk,\cert)$:] $ $
\begin{itemize}
    \item Parse $\vk=\TPRF.\vk$.
    \item Output the outcome of $\TPRF.\Vrfy(\TPRF.\vk,\cert)$.
\end{itemize}
\end{description}


%\protocol
%{Circuit $D[\SKE.\sk,b]$}
%{The description of $D[\SKE.\sk,b]$}
%{fig:description-D}
%{
%\begin{description}
%\setlength{\parskip}{0.3mm} % between paragraph
%\setlength{\itemsep}{0.3mm} % between items
%\item[Constants:] A SKE key $\SKE.\sk$ and a bit $b\in\bit$.
%\item[Input:] A string $\prfinp \in \zo{\inplen}$.
%\end{description}
%\begin{enumerate}
%\item Compute $\beta \lrun \SKE.\Dec(\SKE.\sk,\prfinp)$.
%\item If $\beta\ne \bot$, do the following
%\begin{enumerate}
%\item If $\beta=b$, output $0$. Otherwise, output $1$.
%\end{enumerate}
%\item Otherwise, output $0$.
%\end{enumerate}
%}


The evaluation correctness and the verification correctness of $\PRFSKL$ directly follow from those of $\TPRF$.

\begin{theorem}\label{thm:PRFSKL-from-TPRF}
Suppose $\TPRF$ satisfies extractability on Hadamard basis position and quantum simulatability on computational basis position.
Then, $\PRFSKL$ satisfies strong PR-KLA security.
\end{theorem}
\begin{proof}
Let $\gamma\in[0,1]$ and $\qA$ be a QPT adversary against the strong PR-SKL security of $\PRFSKL$.
We below let $\TPRF.\Ext$ and $\TPRF.\Sim$ be the extraction algorithm and the simulation algorithm that are guaranteed to exist by the security notion of $\TPRF$.
We consider the following three experiments.

\begin{description}
\item[$\hybi{0}$:] This is $\expc{\PRFSKL,\qA}{s}{pr}{kla}(1^\secp,\gamma)$. The detailed description is as follows.
\begin{enumerate}
            \item  The challenger generates $x,\theta\gets\bit^n$, $\TPRF.\msk\gets\TPRF.\KG(1^\secp,1^{n+1})$, $\TPRF.\qsk\gets\TPRF.\qQKG(\allowbreak\TPRF.\msk,\ket{x_\theta}\tensor\ket{0})$, and $\TPRF.\vk\gets\TPRF.\VKG(\TPRF.\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta)$\mor{$\theta\|0$?}, and sends $\qsk\seteq\TPRF.\qsk$ to $\qA$ and sets $\vk\seteq\TPRF.\vk$. 
            \item $\qA$ outputs a classical string $\cert$ and a quantum program with classical input and output $(\ket{\psi},\mat{U})$ whose first register (i.e., output register) is $\bbC^2$ and $\mat{U}$ is a compact classical description of $\{\mat{U}_{\vk^\prime,\prfinp,\prfout}\}_{\vk^\prime,\prfinp,\prfout}$. 


\item Let $D$ be the following distribution.
\begin{description}
\item[$D$:]Generate $\beta\gets\bit$, $\prfinp\gets\Domprf$, $\prfout_0\gets\TPRF.\Eval(\TPRF.\msk,\prfinp)$, and $\prfout_1\gets\Ranprf$. Output $(\beta,\prfinp,\prfout_\beta)$.
\end{description}
Also, let $\cP^\vk=(\mat{P}^\vk_{\beta,\prfinp,\prfout},\mat{Q}^\vk_{\beta,\prfinp,\prfout})_{\beta,\prfinp,\prfout}$ be a collection of binary outcome projective measurements defined in exactly the same way as \cref{def:strong-PR-KLA}, and let $\cP^\vk_D=(\mat{P}^\vk_D,\mat{Q}^\vk_D)$ be the mixture of $\cP^\vk$ with respect to $D$.
Then, the challenger applies $\projimp(\mat{P}^\vk_{D})$ to $\ket{\psi}$ and obtains $p$.
If $\TPRF.\Vrfy(\TPRF.\vk,\cert)=\top$ and $p> \frac{1}{2}+\gamma$, the challenger outputs $1$.
Otherwise, the challenger outputs $0$.
 \end{enumerate}
 \end{description}
 
 We below let $\AccVrfy$ be the event that $\TPRF.\Vrfy(\TPRF.\vk,\cert)=\top$.
 Below, we let $\epsilon=\frac{\gamma}{9}$, $\delta=2^{-\secp}$, and $D_{i}$ be the distribution that outputs $(\beta,\prfinp,\prfout)\gets\TPRF.\Sim(\TPRF.\msk,i)$ for every $i\in[n+1]$. 
 
 \begin{description}
 \item[$\hybi{1}$:] This is the same as $\hybi{0}$ except that the challenger applies $\API_{\cP^\vk,D_{n+1}}^{\epsilon,\delta}$ to $\ket{\psi}$, obtains $\tlp_{n+1}$, and outputs $1$ if and only if $\TPRF.\Vrfy(\TPRF.\vk,\cert)=\top$ and $\tlp_{n+1}> \frac{1}{2}+\gamma-4\epsilon$.
 \end{description}
 

 
From \cref{thm:api_property}, we have
\begin{align}
\Pr[\API_{\cP^\vk,D}^{\epsilon,\delta}\ket{\psi}\ge \frac{1}{2}+\gamma-\epsilon ~\land~ \AccVrfy]
&\ge
\Pr[\projimp(\cP^\vk_D)\ket{\psi}\ge \frac{1}{2}+\gamma ~\land~ \AccVrfy]\\
&=\Pr[\hybi{0}=1]
\label{eqn:projimp-api-D}
\end{align}
\mor{$(\ket{\psi})$?}

We then consider the following QPT sampling algorithm $\Sample$.
\begin{description}
\item[$\Sample(1^\secp)$:] $ $
\begin{itemize}
    \item Generate $x,\theta\gets\bit^n$, $\TPRF.\msk\gets\TPRF.\KG(1^\secp,1^{n+1})$, $\TPRF.\qsk\gets\TPRF.\qQKG(\allowbreak\TPRF.\msk,\ket{x_\theta}\tensor\ket{0})$, and $\TPRF.\vk\gets\TPRF.\VKG(\TPRF.\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta)$.\mor{$\theta\|0$?}
    \item Execute $\qA(\TPRF.\qsk)$ and obtain $\cert$ and $(\ket{\psi},\mat{U})$.
    \item If $\TPRF.\Vrfy(\TPRF.\vk,\cert)=\top$, output $(D,D_{n+1},\cP^\vk,\ket{\psi})$. 
    \takashi{What does it mean to output a distribution?}
    Otherwise, output $(\bot,\bot,\bot,\bot)$.
\end{itemize}
\end{description}
By the quantum simulatability on computational basis position of $\TPRF$, for any QPT $\qA$, we have
\begin{align}
\abs{
\Pr
\left[
\qA(1^\secp,(\beta,\prfinp,\prfout),\cP^\vk,\ket{\psi})=1
\right]-
\Pr
\left[
\qA(1^\secp,(\beta_{n+1},\prfinp_{n+1},\prfout_{n+1}),\cP^\vk,\ket{\psi})=1
\right]
}
=\negl(\secp),
\end{align}
where $(D,D_{n+1},\cP^\vk,\ket{\psi})\gets\Sample(1^\secp)$, $(\beta,\prfinp,\prfout)\gets D$, and $(\beta_{n+1},\prfinp_{n+1},\prfout_{n+1})\gets D_{n+1}$.

Then, from \cref{cor:cind_sample_api}, we have
\begin{align}
\Pr[\hybi{1}=1]=
&\Pr_{
(D,D_{n+1},\cP^\vk,\ket{\psi})\gets\Sample(1^\secp)
}
\left[
\API_{\cP^\vk,D_{n+1}}^{\epsilon,\delta}\ket{\psi}\ge \frac{1}{2}+\gamma-4\epsilon
\right]\\
&\ge
\Pr_{
(D,D_{n+1},\cP^\vk,\ket{\psi})\gets\Sample(1^\secp)
}
\left[
\API_{\cP^\vk,D}^{\epsilon,\delta}\ket{\psi}\ge \frac{1}{2}+\gamma-\epsilon
\right]
- \negl(\secp).
\label{eqn:api-DDn+1}
\end{align}
By combining \cref{eqn:projimp-api-D} and \cref{eqn:api-DDn+1}, we obtain $\Pr[\hybi{1}=1]\ge\Pr[\hybi{0}=1]-\negl(\secp)$.


 \begin{description}
 \item[$\hybi{2}$:] This is the same as $\hybi{1}$ except that the challenger generates $\vk$ as $\vk\gets\TPRF.\VKG(\msk,(x_i^\prime)_{i\in[n]:\theta[i]=1},\theta\|0)$, where $(x_i^\prime)_{i\in[n]:\theta[i]=1}\gets\TPRF.\Ext(\TPRF.\msk,\theta\|0,\cert)$. Note that $\vk$ is needed only after $\qA$ outputs $\cert$.
 \end{description}
 If $\TPRF.\Vrfy(\vk,\cert)=\top$, we have $x_i^\prime=x[i]$ for every $i\in[n]$ such that $\theta[i]=1$, where $(x_i^\prime)_{i\in[n]:\theta[i]=1}\gets\TPRF.\Ext(\TPRF.\msk,\theta\|0,\cert)$.
 Thus, conditioned that $\TPRF.\Vrfy(\vk,\cert)=\top$, $\vk$ distributes identically between $\hybi{1}$ and $\hybi{2}$.
 Therefore, we have $\Pr[\hybi{1}=1]=\Pr[\hybi{2}=1]$.
 
 \medskip

Using, $\qA$, we construct the following adversary $\qB=(\qB_0,\qB_1,\qB_2)$ that attacks the strong monogamy of entanglement property of BB84 states.
\begin{description}
\item[$\qB_0$:] Given an $n$-qubit BB84 state $\ket{\phi}$, $\qB_0$ first generates $\TPRF.\msk\gets\TPRF.\KG(1^\secp,1^{n+1})$ and $\TPRF.\qsk\gets\TPRF.\qQKG(\TPRF.\msk,\ket{\phi}\tensor\ket{0})$.
$\qB_0$ then sends $\qsk\seteq\TPRF.\qsk$ to $\qA$.  When $\qA$ outputs a classical string $\cert$ and a quantum program with classical input and output $(\ket{\psi},\mat{U})$, 
$\qB_0$ sends $(\TPRF.\msk,\cert,(\ket{\psi},\mat{U}))$ to $\qB_1$ and $(\TPRF.\msk,\cert)$ to $\qB_2$.
\item[$\qB_1$:] Given $\theta$ and $(\TPRF.\msk,\cert,(\ket{\psi},\mat{U}))$, $\qB_1$ first computes $(x^\prime_i)_{i\in[n]:\theta[i]=1}\gets\TPRF.\Ext(\TPRF.\msk,\theta\|0,\cert)$ and $\vk\gets\TPRF.\VKG(\TPRF.\msk,(x^\prime_i)_{i\in[n]:\theta[i]=1},\theta\|0)$.
$\qB_1$ applies $\API_{\cP^\vk,D_{n+1}}^{\epsilon,\delta}$ to $\ket{\psi}$ and obtains the outcome $\tlp_{n+1}$ and post state $\ket{\tlpsi_1}$.
If $\tlp_{n+1}<\frac{1}{2}+\gamma-4\epsilon$, $\qB_1$ aborts.
Otherwise, $\qB_1$ does the following from $i=1$ to $i=n$.
\begin{itemize}
\item If $\theta[i]=1$, set ${\tlpsi_{i+1}}\seteq\ket{\tlpsi_i}$ and go to the $i+1$-th loop. Otherwise, do the following.
\item Apply $\API_{\cP^\vk,D_i}^{\epsilon,\delta}$ to $\ket{\tlpsi_i}$ and obtain the result $\tlp_i$ and the post state $\ket{\tlpsi_i^\prime}$.
\item Set $x_{i}^\prime\seteq0$ if $\tlp_i>\frac{1}{2}$ and otherwise $x_{i}\seteq1$.
\item Uncompute the previous steps and obtain a state $\ket{\tlpsi_{i+1}}$.
\end{itemize}
$\qB_1$ outputs $(x_i^\prime)_{i\in[n]:\theta[i]=0}$.
\item[$\qB_2$:]Given $\theta$ and $(\TPRF.\msk,\cert)$, $\qB_2$ outputs $(x^\prime_i)_{i\in[n]:\theta[i]=1}\gets\TPRF.\Ext(\TPRF.\msk,\theta\|0,\cert)$.
\end{description}

$\qB_1$ perfectly simulates $\hybi{2}$ and obtain $\tlp_{n+1}$ and $\cert$ that distribute in exactly the same way as $\hybi{1}$.
We prove that if the output of the simulated $\hybi{2}$ is equal to $1$, that is, we have $\tlp_{n+1}\ge\frac{1}{2}+\gamma-4\epsilon$ and $\TPRF.\Vrfy(\TPRF.\vk,\cert)=\top$, $\qB$ wins the experiment. We can immediately conclude that if $\TPRF.\Vrfy(\TPRF.\vk,\cert)=\top$, we have $x^\prime_i=x[i]$ for every $i\in[n]$ such that $\theta[i]=1$, from the extractability on Hadamard basis position.
We below show that if $\qA$ wins in the simulated $\hybi{2}$, we also have $x^\prime_i=x[i]$ with overwhelming probability for every $i\in[n]$ such that $\theta[i]=0$, from the simulatability on computational basis position.

Let $i_1$ be the smallest index in $[n]$ such that $\theta[i_1]=0$.
We prove that $x^\prime_{i_1}=x[i_1]$ with overwhelming probability.
We first assume $x[i_1]=0$.
From \cref{thm:api_property}, we have $\Pr[\abs{\tlp_{n+1}-\API_{\cP,D_{n+1}}^{\epsilon,\delta}(\tlrho_1)}\le\epsilon]=1-\negl(\secp)$.
This means we have
\begin{align}
\Pr\left[\API_{\cP,D_{n+1}}^{\epsilon,\delta}(\tlrho_1)\ge\frac{1}{2}+\gamma-5\epsilon  ~\middle |~ \hybi{2}=1\right]=1-\negl(\secp).
\label{eqn:api-Dn+1projective}
\end{align}
We then consider the following QPT sampling algorithm $\Sample$.
\begin{description}
\item[$\Sample_{n+1,i_1}(1^\secp)$:] $ $
\begin{itemize}
    \item Generate $x,\theta\gets\bit^n$, $\TPRF.\msk\gets\TPRF.\KG(1^\secp,1^{n+1})$, and $\TPRF.\qsk\gets\TPRF.\qQKG(\allowbreak\TPRF.\msk,\ket{x_\theta}\tensor\ket{0})$.
    \item Execute $\qA(\TPRF.\qsk)$ and obtain $\cert$ and $(\ket{\psi},\mat{U})$.
    \item Compute $(x^\prime_i)_{i\in[n]:\theta[i]=1}\gets\TPRF.\Ext(\TPRF.\msk,\theta\|0,\cert)$ and $\vk\gets\TPRF.\VKG(\TPRF.\msk,(x^\prime_i)_{i\in[n]:\theta[i]=1},\theta\|0)$.
    \item Apply $\API_{\cP^\vk,D_{n+1}}^{\epsilon,\delta}$ to $\rho$ and obtain the outcome $\tlp_{n+1}$ and the post state $\ket{\tlpsi_1}$.
    \item If $\TPRF.\Vrfy(\vk,\cert)=\top$ and $\tlp_{n+1}\ge\frac{1}{2}+\gamma-4\epsilon$, output $(D_{n+1},D_{i_1},\cP^\vk,\ket{\tlpsi_1})$. Otherwise, output $(\bot,\bot,\bot,\bot)$.
\end{itemize}
\end{description}
$\Sample_{n+1,i_1}$ aborts if $\TPRF.\Vrfy(\vk,\cert)=\bot$. Thus, if it compute $\vk$ as $\vk\gets\TPRF.\VKG(\TPRF.\msk,(x[i])_{i\in[n]:\theta[i]=1},\theta\|0)$, the output distribution of $\Sample_{n+1,i_1}$ does not change.
Then, by the quantum simulatability on computational basis position of $\TPRF$, for any QPT $\qA$, we have
\begin{align}
\abs{
\Pr
\left[
\qA(1^\secp,(\beta_{n+1},\prfinp_{n+1},\prfout_{n+1}),\cP^\vk,\ket{\tlpsi_1})=1
\right]
-
\Pr
\left[
\qA(1^\secp,(\beta_{i_1},\prfinp_{i_1},\prfout_{i_1}),\cP^\vk,\ket{\tlpsi_1})=1
\right]
}
=\negl(\secp),
\end{align}
where $(D_{n+1},D_{i_1},\cP^\vk,\ket{\tlpsi_1})\gets\Sample_{n+1,i_1}(1^\secp)$, $(\beta_{n+1},\prfinp_{n+1},\prfout_{n+1})$, and $(\beta_{i_1},\prfinp_{i_1},\prfout_{i_1})\gets D_{i_1}$.
We note that the application of $\API_{\cP^\vk,D_{n+1}}^{\epsilon,\delta}$ can be simulated by the quantum access to the map
\begin{align}
\ket{r}\ket{t}\ra\ket{r}\ket{t\oplus\TPRF.\Sim(\TPRF.\msk,n+1;r)}
\end{align}
provided in the security experiment of quantum simulatability on computational basis position.
Then, from \cref{cor:cind_sample_api}, we have
\begin{align}
&\Pr
\left[
\API_{\cP,D_{i_1}}^{\epsilon,\delta}(\tlrho_1)\ge \frac{1}{2}+\gamma-8\epsilon
\right]\\
&\ge
\Pr
\left[
\API_{\cP,D_{n+1}}^{\epsilon,\delta}(\tlrho_1)\ge \frac{1}{2}+\gamma-5\epsilon
\right]
- \negl(\secp),
\label{eqn:api-Dn+1Di_1}
\end{align}
where $(D_{n+1},D_{i_1},\cP^\vk,\ket{\tlpsi_1})\gets\Sample_{n+1,i_1}(1^\secp)$.
$\Sample_{n+1,i_1}$ simulates $\hybi{2}$ and aborts if the output of simulated $\hybi{2}$ is not equal to $1$.
Thus, we have
\begin{align}
\Pr
\left[
\API_{\cP,D_{i_1}}^{\epsilon,\delta}(\tlrho_1)\ge \frac{1}{2}+\gamma-8\epsilon
\middle | \hybi{2}=1
\right]
\ge
\Pr
\left[
\API_{\cP,D_{n+1}}^{\epsilon,\delta}(\tlrho_1)\ge \frac{1}{2}+\gamma-5\epsilon
\middle | \hybi{2}=1
\right]
- \negl(\secp),
\label{eqn:api-Dn+1Di_1-conditioned}
\end{align}
where $(D_{n+1},D_{i_1},\cP^\vk,\ket{\tlpsi_1})\gets\Sample_{n+1,i_1}(1^\secp)$.
By combining it with \cref{eqn:api-Dn+1projective}, we obtain
\begin{align}
&\Pr
\left[
\API_{\cP,D_{i_1}}^{\epsilon,\delta}(\tlrho_1)\ge \frac{1}{2}+\gamma-8\epsilon
\middle | \hybi{2}=1
\right]
\ge
1-\negl(\secp).
\end{align}
This means $x_{i_1}^\prime=x[i_1]=0$ holds with overwhelming probability in this case if the output of $\hybi{2}$ simulated by $\qB$ is equal to $1$.


We next assume $x[i_1]=1$.
We define $\Drev_{n+1}$ as the distribution that generates $(\beta,\prfinp,\prfout)\gets D_{n+1}$ and outputs $(1\oplus\beta,\prfinp,\prfout)$.
Then, for any random coin $r$, we have $(\mat{P}^{\vk}_{\Drev_{n+1}(r)},\mat{Q}^{\vk}_{\Drev_{n+1}(r)})=(\mat{Q}^{\vk}_{\D_{n+1}(r)},\mat{P}^{\vk}_{\D_{n+1}(r)})$ since we have $\mat{Q}^{\vk}_{\beta,\prfinp,\prfout}=\mat{I}-\mat{P}^{\vk}_{\beta,\prfinp,\prfout}=\mat{P}^{\vk}_{1\oplus \beta,\prfinp,\prfout}$ for any tuple $(\beta,\prfinp,\prfout)$.
Therefore, $ \API_{\cP^\vk,\Drev_{n+1}}^{\epsilon ,\delta}$ is exactly the same process as  $\API_{\cPrev^{\vk},D_{n+1}}^{\epsilon ,\delta}$, where $\cPrev^{\vk}=(\mat{Q}^{\vk}_{\beta,\prfinp,\prfout},\mat{P}^{\vk}_{\beta,\prfinp,\prfout})_{\beta,\prfinp,\prfout}$.
From \cref{thm:api_property}, we have $\Pr[\abs{(1-\tlp_{n+1})-\API_{\cP,D_{n+1}}^{\epsilon,\delta}(\tlrho_1)}\le\epsilon]=1-\negl(\secp)$.
This means we have
\begin{align}
\Pr\left[\API_{\cP,D_{n+1}}^{\epsilon,\delta}(\tlrho_1)\le\frac{1}{2}-\gamma+5\epsilon  ~\middle |~ \hybi{2}=1\right]=1-\negl(\secp).
\label{eqn:api-Dn+1revprojective}
\end{align}
We then define $\Samplerev_{n+1,i_1}$ as a QPT sampling algorithm that behaves in the same way as $\Sample_{n+1,i_1}$ except that it outputs $(\Drev_{n+1},D_{i+1},\cP^\vk,\ket{\tlpsi_1})$ if $\tlp_{n+1}\ge\frac{1}{2}+\gamma-4\epsilon$ holds.
For any QPT $\qA$, we have
\begin{align}
\abs{
\Pr
\left[
\qA(1^\secp,(\beta_{n+1},\prfinp_{n+1},\prfout_{n+1}),\cP^\vk,\ket{\tlpsi_1})=1
\right]
-
\Pr
\left[
\qA(1^\secp,(\beta_{i_1},\prfinp_{i_1},\prfout_{i_1}),\cP^\vk,\ket{\tlpsi_1})=1
\right]
}
=\negl(\secp),
\end{align}
where $(\Drev_{n+1},D_{i_1},\cP^\vk,\ket{\tlpsi_1})\gets\Samplerev_{n+1,i_1}(1^\secp)$, $(\beta_{n+1},\prfinp_{n+1},\prfout_{n+1})\gets \Drev_{n+1}$, and $(\beta_{i_1},\prfinp_{i_1},\prfout_{i_1})\gets D_{i_1}$.
This is bacause both $\Drev_{n+1}$ and $D_{i+1}$ are computationally indistinguishable from $\Drev$ that generates $(\beta,\prfinp,\prfout)\gets D$ and outputs $(1\oplus\beta,\prfinp,\prfout)$ from the quantum simulatabality on computational basis of $\TPRF$.
Then, from \cref{cor:cind_sample_api}, we have
\begin{align}
\Pr
\left[
\API_{\cP,D_{i_1}}^{\epsilon,\delta}(\tlrho_1)\le \frac{1}{2}-\gamma+8\epsilon
\right]
\ge
\Pr
\left[
\API_{\cP,\Drev_{n+1}}^{\epsilon,\delta}(\tlrho_1)\le \frac{1}{2}-\gamma+5\epsilon
\right]
- \negl(\secp),
\label{eqn:api-Drevn+1Di_1}
\end{align}
where $(\Drev_{n+1},D_{i_1},\tlrho_1)\gets\Samplerev_{n+1,i_1}(1^\secp)$.
$\Sample_{n+1,i_1}$ simulates $\hybi{2}$ and aborts if the output of simulated $\hybi{2}$ is not equal to $1$.
Thus, we have
\begin{align}
\Pr
\left[
\API_{\cP,D_{i_1}}^{\epsilon,\delta}(\tlrho_1)\le \frac{1}{2}-\gamma+8\epsilon
\middle | \hybi{2}=1
\right]
\ge
\Pr
\left[
\API_{\cP,\Drev_{n+1}}^{\epsilon,\delta}(\tlrho_1)\ge \frac{1}{2}-\gamma+5\epsilon
\middle | \hybi{2}=1
\right]
- \negl(\secp),
\label{eqn:api-Drevn+1Di_1-conditioned}
\end{align}
where $(\Drev_{n+1},D_{i_1},\tlrho_1)\gets\Samplerev_{n+1,i_1}(1^\secp)$.
By combining it with \cref{eqn:api-Dn+1revprojective}, we obtain
\begin{align}
&\Pr
\left[
\API_{\cP,D_{i_1}}^{\epsilon,\delta}(\tlrho_1)\le \frac{1}{2}-\gamma+8\epsilon
\middle | \hybi{2}=1
\right]
\ge
1-\negl(\secp),
\end{align}
where $(\Drev_{n+1},D_{i_1},\tlrho_1)\gets\Samplerev_{n+1,i_1}(1^\secp)$.
This means $x_{i_1}^\prime=x[i_1]=1$ holds with overwhelming probability in this case the output of $\hybi{2}$ simulated by $\qB$ is equal to $1$.

From the above, $x_{i_1}^\prime=x[i_1]$ holds regardless of the value of $x[i_1]$ with overwhelming probability.
This means $\ket{\tlpsi_2}$ that is obtained by uncomputing the extraction process of $x_{i_1}^\prime$ from $\ket{\tlpsi_1}$ is negligibly close to $\ket{\tlpsi_1}$.
Then, we can similarly prove that $x_i^\prime=x[i]$ holds with overwhelming probability for every $i\in[n]$ such that $\theta[i]=0$ if the output of $\hybi{2}$ simulated by $\qB$ is equal to $1$.

From the above discussions, we have $\Pr[\hybi{2}=1]\le\Pr[\SMoEBB(\qB,n)=1]$.
Thus, from the strong monogamy of entanglement property of BB84 states, we have $\Pr[\hybi{2}=1]=\negl(\secp)$.
This completes the proof.
\end{proof}


\input{const-TPRF-BB84}





==> const-TPRF-BB84.tex <==
% !TEX root = main.tex

\newcommand{\simsk}{\hat{\sk}}

\subsection{Construction of Tailored PRF for BB84 state}\label{sec:const-TPRF-BB84}
We construct Tailored PRF scheme for BB84 state $\TPRF=(\TPRF.\KG,\TPRF.\qQKG, \TPRF.\Eval, \TPRF.\qQEval,\TPRF.\qDel,\allowbreak\TPRF.\Vrfy)$.
We use the following building blocks.
\begin{itemize}
\item A SKE scheme $\SKE=\SKE.(\E,\D)$ with ciphertext pseudorandomness.
\item A constrained PRF scheme $\CPRF=\CPRF.(\Setup,\Constrain,\Eval,\CEval)$.
\end{itemize}

\begin{description}
\item[$\TPRF.\KG(1^\secp,1^n)$:] $ $
\begin{itemize}
    \item Generate $\SKE.\sk_i\gets \bit^\secp$ for every $i\in [n]$.
    \item Generate $\CPRF.\msk_i\gets \CPRF.\Setup(1^\secp)$ for every $i\in [n]$.
    \item Generate $\CPRF.\sk_{i,b}\gets\CPRF.\Constrain(\msk_i,D[\SKE.\sk_i,b])$ for every $i\in[n]$ and $b\in\bit$, where the circuit $D$ is described in \cref{fig:description-D}.
%    \item Generate
%    \begin{align}
%    \qsk_i\seteq
%    \begin{cases}
%    \ket{x[i]}\ket{\CPRF.\sk_{i,x[i]}} & (\textrm{if~}\theta[i]=0)\\
%    \frac{1}{\sqrt{2}}\left(\ket{0}\ket{\CPRF.\sk_{i,0}}+(-1)^{x[i]}\ket{1}\ket{\CPRF.\sk_{i,1}}\right) & (\textrm{if~}\theta[i]=1)
%    \end{cases}
%    \end{align}
%    for every $\in[n]$.
    \item Output $\msk\seteq ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$.
\end{itemize}

\item[$\TPRF.\qQKG(\msk,\ket{\psi_1}\tensor\cdots\tensor\ket{\psi_n})$:] $ $
\begin{itemize}
\item Parse $\msk= ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$.
\item Let $U_i$ be the unitary that maps $\ket{u}\ket{v}$ to $\ket{u}\ket{v\oplus\CPRF.\sk_{i,u}}$.
\item Apply $U_i$ to $\ket{\psi_i}\ket{0\cdots0}$ and obtain $\qsk_i$ for every $i\in[n]$.
\item Output $\qsk\seteq(\qsk_1,\ldots,\qsk_n)$.
\end{itemize}

\item[$\TPRF.\VKG(\msk,(x_i)_{i\in[n]:\theta[i]=1},\theta)$:] $ $
\begin{itemize}
\item Parse $\msk= ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$.
\item Output $\vk\seteq((x_i)_{i\in[n]:\theta[i]=1},\theta,(\CPRF.\sk_{i,0},\CPRF.\sk_{i,1})_{i\in[n],\theta[i]=1})$.
\end{itemize}


\item[$\TPRF.\Eval(\msk,\prfinp)$:] $ $
\begin{itemize}
    \item Parse $\msk= ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$. 
    \item Generate $\cprfout_i\gets \CPRF.\CEval(\CPRF.\sk_{i,0},\prfinp)$ for every $i\in [n]$.
\item Output $\prfout\seteq\bigoplus_{i\in[n]}\cprfout_i$. 
\end{itemize}
 
\item[$\TPRF.\qQEval(\qsk,\prfinp)$:] $ $
\begin{itemize}
   \item Parse  $\qsk= (\qsk_1,\ldots,\qsk_n)$.
   \item Let $E_i$ be the unitary that maps $\ket{u}\ket{\CPRF.\sk}\ket{v}$ to $\ket{u}\ket{\CPRF.\sk}\ket{v\oplus\CPRF.\CEval(\CPRF.\sk,s)}$ for every $i\in[n]$.
   \item Apply $E_i$ to $\qsk_i\tensor\ket{0\cdots0}$, measure the last register, and obtain $\cprfout_i^\prime$ for every $i\in[n]$.
\item Output $\cprfout^\prime\seteq\bigoplus_{i\in[n]}\cprfout_i^\prime$. 
\end{itemize}

\item[$\TPRF.\qDel(\qsk)$:] $ $
\begin{itemize}
\item Parse $\qsk= (\qsk_1,\ldots,\qsk_n)$.
\item Measure $\qsk_i$ in Hadamard basis and obtain $(e_i,d_i)$ for every $i\in[n]$.
\item Output $\cert\seteq (e_i,d_i)_{i\in[n]}$.
\end{itemize}


\item[$\TPRF.\Vrfy(\vk,\cert)$:] $ $
\begin{itemize}
    \item Parse $\vk=((x_i)_{i\in[n]:\theta[i]=1},\theta,(\CPRF.\sk_{i,0},\CPRF.\sk_{i,1})_{i\in[n],\theta[i]=1})$ and $\cert=(e_i,d_i)_{i\in[n]}$.
    \item Output $\top$ if $e_i=x[i] \oplus d_i\cdot(\CPRF.\sk_{i,0}\oplus\CPRF.\sk_{i,1})$ holds for every $i\in[n]$ such that $\theta[i]=1$. Otherwise, output $\bot$.
\end{itemize}
\end{description}


\protocol
{Circuit $D[\SKE.\sk,b]$}
{The description of $D[\SKE.\sk,b]$}
{fig:description-D}
{
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Constants:] A SKE key $\SKE.\sk$ and a bit $b\in\bit$.
\item[Input:] A string $\prfinp \in \zo{\inplen}$.
\end{description}
\begin{enumerate}
\item Compute $\beta \lrun \SKE.\Dec(\SKE.\sk,\prfinp)$.
\item If $\beta\ne \bot$, do the following
\begin{enumerate}
\item If $\beta=b$, output $0$. Otherwise, output $1$.
\end{enumerate}
\item Otherwise, output $0$.
\end{enumerate}
}




\paragraph{Evaluation Correctness.}
Fix $x,\theta\in\bit^n$ and $\prfinp\in\bit^\inplen$.
We show that $\prfout_i^\prime=\CPRF(\msk_i,s)$ holds with overwhelming probability for $\prfout_i^\prime$ computed in $\TPRF.\qQEval(\qsk,s)$ for every $i\in[n]$, where $\msk\gets\TPRF.\KG(1^\secp,1^n)$ and $(\qsk_1,\ldots,\qsk_n)\gets\TPRF.\qQKG(\msk,\ket{x_\theta})$.

We first consider $i\in[n]$ such that $\theta[i]=0$. In this case, $\qsk_i=\ket{x[i]}\ket{\CPRF.\sk_{i,x[i]}}$.
Thus, the state obtained by applying the map $E_i$ to $\qsk_i\tensor\ket{0\cdots0}$ is $\ket{x[i]}\ket{\CPRF.\sk_{i,x[i]}}\ket{\CPRF.\CEval(\CPRF.\sk_{i,x[i]},\prfinp)}$, and thus $\cprfout_i^\prime=\CPRF.\Eval(\CPRF.\sk_{i,x[i]},\prfinp)$.
From the sparseness of $\SKE$, $\SKE.\Dec(\SKE.\sk_i,\prfinp)=\bot$ holds with overwhelming probability.
Therefore, we have $\cprfout_i^\prime=\CPRF.\CEval(\CPRF.\sk_{i,b},\prfinp)=\CPRF.\Eval(\CPRF.\msk_i,\prfinp)$, as we want.

We next consider $i\in[n]$ such that $\theta[i]=1$. In this case, $\qsk_i=\frac{1}{\sqrt{2}}(\ket{0}\ket{\CPRF.\sk_{i,0}}+(-1)^{x[i]}\ket{1}\ket{\CPRF.\sk_{i,1}})$.
Thus, the state obtained by applying the map $E_i$ to $\qsk_i\tensor\ket{0\cdots0}$ is 
\begin{align}
\frac{1}{\sqrt{2}}(\ket{0}\ket{\CPRF.\sk_{i,0}}\ket{\CPRF.\CEval(\CPRF,\sk_{i,0},\prfinp)}+(-1)^{x[i]}\ket{1}\ket{\CPRF.\sk_{i,1}}\ket{\CPRF.\CEval(\CPRF.\sk_{i,1},\prfinp)})
\end{align}
From the sparseness of $\SKE$, $\SKE.\Dec(\SKE.\sk_i,\prfinp)=\bot$ holds with overwhelming probability.
Thus, we have $\CPRF.\CEval(\CPRF.\sk_{i,0},\prfinp)=\CPRF.\CEval(\CPRF.\sk_{i,1},\prfinp)=\CPRF.\Eval(\CPRF.\msk_i,\prfinp)$.
Therefore, we have $\cprfout_i^\prime=\CPRF.\Eval(\CPRF.\msk_i,\prfinp)$ with overwhelming probability, as we want.



\paragraph{Verification Correctness.}
We omit the proof of the verification correctness of $\PRFSKL$ since it is almost the same as that for $\PKESKL$ presented in \cref{sec:const-PKE-SKL-classical-certificate}.
%We show that $e_i=x[i]\oplus d_i \cdot (\PKE.\dk_{i,0}\oplus\PKE.\dk_{i,1})$ holds for every $(e_i,d_i)$ for $i\in[n]$ such that $\theta[i]=1$ obtained when executing $\SKL.\qDel(\qdk)$, where $(\ek,\qdk,\vk)\gets\SKL.\qKG(1^\secp)$.
%For every $i\in[n]$ such that $\theta[i]=1$, we have $\qdk_i=\frac{1}{\sqrt{2}}(\ket{0}\ket{\PKE.\dk_{i,0}}+(-1)^{x[i]}\ket{1}\ket{\PKE.\dk_{i,1}})$.
%If we apply Hadamard gate to every qubit of $\qdk_i$, we obtain
%\begin{align}
%&\frac{1}{\sqrt{2}}\left(
%\frac{1}{\sqrt{2^{\ell+1}}}\sum_{e_i,d_i} (-1)^{d_i\cdot\PKE.\dk_{i,0}}\ket{e_i}\ket{d_i}
%+
%\frac{1}{\sqrt{2^{\ell+1}}}\sum_{e_i,d_i} (-1)^{x[i]\oplus e_i\oplus d_i\cdot\PKE.\dk_{i,1}}\ket{e_i}\ket{d_i}
%\right)\\
%=&
%\frac{1}{\sqrt{2^{\ell}}}\sum_{e_i,d_i:d_i\cdot\PKE.\dk_{i,0}=x[i]\oplus e_i\oplus d_i\cdot\dk_{i,1}}(-1)^{d_i\cdot\PKE.\dk_{i,0}}\ket{e_i}\ket{d_i}.
%\end{align}
%Thus, we have $e_i=x[i]\oplus d_i \cdot (\PKE.\dk_{i,0}\oplus\PKE.\dk_{i,1})$ for $(e_i,d_i)$ for every $i\in[n]$ such that $\theta[i]=1$.

\begin{theorem}\label{thm:TPRF-ext-hbp}
$\TPRF$ satisfies extractability on Hadamard basis position.
\end{theorem}
\begin{proof}
We first describe $\TPRF.\Ext$.
\begin{description}
\item[$\TPRF.\Ext(\msk,\theta,\cert)$:] $ $
\begin{itemize}
    \item Parse $\msk= ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$ and $\cert=(e_i,d_i)_{i\in[n]}$.
    \item Compute $x_i^\prime=e_i \oplus d_i\cdot(\CPRF.\sk_{i,0}\oplus\CPRF.\sk_{i,1})$ for every $i\in[n]$ such that $\theta[i]=1$.
    \item Output $(x_i^\prime)_{i\in[n]:\theta[i]=1}$.
\end{itemize}
\end{description}

Fix $x,\theta\in\bit^n$, $\msk=((\CPRF.\msk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})\gets\KG(1^\secp,1^n)$, and a string $\cert=(e_i,d_i)_{i\in[n]}$ such that $\TPRF.\Vrfy(x,\theta,\msk,\cert)=\top$.
We have $e_i=x[i] \oplus d_i\cdot(\CPRF.\sk_{i,0}\oplus\CPRF.\sk_{i,1})$, that is, $x[i]=e_i \oplus d_i\cdot(\CPRF.\sk_{i,0}\oplus\CPRF.\sk_{i,1})$ for every $i\in[n]$ such that $\theta[i]=1$.
This proves the extractability on Hadamard basis position of $\TPRF$.
\end{proof}


\begin{theorem}\label{thm:TPRF-sim-cbp}
Suppose $\SKE$ is a SKE scheme with ciphertext pseudoranoomness and $\CPRF$  is a selectively single-key private CPRF scheme.
Then, $\TPRF$ satisfies simulatability on computational basis position.
\end{theorem}
\begin{proof}
We first describe $\TPRF.\Sim$.
\begin{description}
\item[$\TPRF.\Sim(\msk,j)$:] $ $
\begin{itemize}
    \item Parse $\msk= ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$.
    \item Generate $\beta\gets\bit$ and $\prfinp\gets\SKE.\Enc(\SKE.\sk_j,\beta)$.
    \item Generate $\cprfout_i\gets\CPRF.\Eval(\CPRF.\msk_i,\prfinp)$ for every $i\in[n]$.
    \item Set $\cprfout\seteq \bigoplus_{i\in[n]}\cprfout_i$.
    \item Output $(\beta,\prfinp,\prfout)$.
\end{itemize}
\end{description}
Let $\qA$ be a QPT adversary against the simulatability on computational basis position of $\TPRF$. 
We consider the following sequence of experiments.
\begin{description}
\item[$\hybi{0}$:] This is $\expb{\TPRF,\Sim,\qA}{sim}{cbp}(1^\secp,\coin=1)$. The detailed description is as follows.
\begin{enumerate}
\item $\qA$ sends $(x,\theta,i^*)$ satisfying $\theta[i^*]=0$ to the challenger. The challenger generates $\SKE.\sk_i\gets\bit^\secp$ and $\CPRF.\msk_i\gets\CPRF.\Setup(1^\secp)$ for every $i\in[n]$, and $\CPRF.\sk_{i,b}\gets\Constrain(\msk_i,D[\SKE.\sk_i,b])$ for every $i\in[n]$ and $b\in\bit$.
The challenger applies $U_i$ to $H^{\theta[i]}\ket{x[i]}\ket{0\cdots0}$ and obtain $\qsk_i$ for every $i\in[n]$, where $U_i$ is the unitary that maps $\ket{u}\ket{v}$ to $\ket{u}\ket{v\oplus\CPRF.\sk_{i,u}}$.
The challenger sets $\msk= ((\CPRF.\msk_i)_{i\in[n]},(\SKE.\sk_i)_{i\in[n]},(\CPRF.\sk_{i,b})_{i\in[n],b\in\bit})$ and $\vk\seteq((x_i)_{i\in[n]:\theta[i]=1},\theta,(\CPRF.\sk_{i,0},\allowbreak\CPRF.\sk_{i,1})_{i\in[n],\theta[i]=1})$, and sends $\qsk\seteq(\qsk_1,\ldots,\qsk_n)$ and $\vk$ to $\qA$.
\item $\qA$ can get access to the following oracle.
\begin{description}
\item[$\Oracle{sim}$:] On input $j\in[n]$, it returns $\TPRF.\Sim(\msk,j)$.
%\item[$\Oracle{eval}$:]It generates $x\gets\Domprf$ and returns $(x,\Eval(\prfk,x))$.\fuyuki{To Do: remove.}
%\item[$\Oracle{ext}$:]On input $(x,y)$, it computes $\prfk^\prime \gets\KeyExtract(\xk,(x,y))$.
%If $\prfk'=\prfk$, it returns special symbol $\challenge$. Otherwise, it returns $\prfk'$.
\end{description}

\item The challenger sends $(\beta^*,\prfinp^*,\prfout^*)$ to $\qA$ generated as follows.
\begin{itemize}
    \item Generate $\beta^*\gets\bit$ and $\prfinp^*\gets\SKE.\Enc(\SKE.\sk_{i^*},\beta^*)$.
    \item Generate $\cprfout_i^*\gets\CPRF.\CEval(\CPRF.\msk_i,\prfinp^*)$ for every $i\in[n]$.
    \item Set $\cprfout^*\seteq \bigoplus_{i\in[n]}\cprfout_i^*$.
    \item Output $(\beta^*,\prfinp^*,\prfout^*)$.
\end{itemize}


\item When $\qA$ terminates with output $\coin^\prime$, the challenger outputs $\coin^\prime$.
\end{enumerate}

\end{description}

Since $\theta[i^*]=0$, we have $\qsk_{i^*}=\ket{x[i^*]}\ket{\CPRF.\sk_{i^*,x[i^*]}}$.
Also, $\vk$ consists of $(\CPRF.\sk_{i,0},\CPRF.\sk_{i,1})_{i\in[n]:\theta[i]=1}$ aside from $(x[i])_{i\in[n]:\theta[i]=1}$ and $\theta$, and $\TPRF.\Sim$ can be executed with the oracle access to $\CPRF.\Eval(\msk_{i^*},\cdot)$.
In other words, to simulate the view of $\qA$ in $\hybi{0}$, we need $\CPRF.\sk_{i^*,x[i^*]}$ and the oracle access to $\CPRF.\Eval(\msk_{i^*},\cdot)$, but not $\CPRF.\sk_{i^*,1-x[i^*]}$.
This allows us to use the single-key security of $i^*$-th instance of $\CPRF$ below.



\begin{description} 
 \item[$\hybi{1}$:] This is the same as $\hybi{0}$ except that if $\beta^\ast\ne x[i^\ast]$, we use $\CPRF.\prfout^\ast_{i^*} \gets \bit^\outlen$ instead of $\CPRF.\prfout^\ast_{i^*} \gets \CPRF.\CEval(\CPRF.\msk_{i^*},\prfinp^\ast)$.
% In addition, we also change $\Oracle{sim}(\iop,i)$ as follows. Letting $\iop=(a,b)$ and $z \seteq \Dec^{\sfout}(\sfout.\sk,b)$, if $z=\ct_{\sfin}$ and $\msg[i]=\gamma$, we use $y \seteq \sfout.\ct \gets \Enc^{\sfout}_{}(\sfout.\pk,\sfin.\ct)$ instead of $y \seteq \sfout.\ct \seteq \Enc^{\sfout}_{}(\sfout.\pk,\sfin.\ct;\prfg(x))$.

Since $D[\SKE.\sk_{i^*},x[i^*]](\prfinp^*)=1$ if $\beta^*\ne x[i^*]$, we have $\abs{\Pr[\hybi{0}=1]-\Pr[\hybi{1}=1]}=\negl(\secp)$ from the selective single-key pseudorandomness of $\CPRF$.

 \item[$\hybi{2}$:] This is the same as $\hybi{1}$ except that we use a simulated $(\stinfo_\Sim,\CPRF.\simsk_{i^*,x[i^*]}) \gets \CPRF.\Sim_1(1^\secp)$ instead of $\CPRF.\sk_{i^*,x[i^*]} \gets \CPRF.\Constrain(\msk_{i^*},D[\SKE.\sk_{i^*},x[i^*]])$ for generating $\qsk_{i^*}$.
 Also, if $\beta^*= x[i^\ast]$, the challenger computes $\CPRF.\prfout^\ast_{i^*} \gets \CPRF.\Sim_2(\stinfo_\Sim,\prfinp^\ast,0)$.
 In addition, we also change the behavior of $\Oracle{sim}$ on input $j\in[n]$ as follows.
 \begin{itemize}
 \item Generate $\beta\gets\bit$, $\prfinp \gets \SKE.\Enc(\SKE.\sk_{j},\beta)$.
 \item Generate $\CPRF.\prfout_{i^*}\gets\CPRF.\Sim_2(\stinfo_\Sim,\prfinp,\alpha)$, where $\alpha=D[\SKE.\sk_{i^*},x[i^*]](\prfinp)$.
 \item Generate $\CPRF.\prfout_i\gets\CPRF.\Eval(\msk_i,\prfinp)$ for every $i\in[n]\setminus\{i^*\}$.
 \item Set $\prfout\seteq\bigoplus_{i\in[n]}\CPRF.\prfout_i$.
 \item Return $(\beta,\prfinp,\prfout)$.
 \end{itemize}

From the selective single-key privacy of $\CPRF$, we have $\abs{\Pr[\hybi{1}=1]-\Pr[\hybi{2}=1]}=\negl(\secp)$.


\item[$\hybi{3}$:] This is the same as $\hybi{2}$ except that we use $\prfinp^\ast \gets \zo{\inplen}$ instead of $\prfinp^\ast \gets \SKE.\Enc(\SKE.\sk_{i^*}, \beta^\ast)$.

By the previous change, $\SKE.\sk_{i^*}$ is used only when generating $\prfinp^*$.
Then, from the ciphertext pseudorandomness of $\SKE$, we have $\abs{\Pr[\hybi{2}=1]-\Pr[\hybi{3}=1]}=\negl(\secp)$

\item[$\hybi{4}$:] This is the same as $\hybi{3}$ except that we undo the change at $\hybi{2}$.

From the selective single-key privacy of $\CPRF$, we have $\abs{\Pr[\hybi{3}=1]-\Pr[\hybi{4}=1]}=\negl(\secp)$.

\item[$\hybi{5}$:] This is the same as $\hybi{3}$ except that if $\beta^*\ne x[i^*]$, $\prfout^*$ is generated as $\prfout^*\gets\bit^\outlen$ instead of $\prfout^*\seteq\bigoplus_{i\in[n]}\CPRF.\prfout_i^*$.

If $\beta^*\ne x[i^*]$, we generate $\CPRF.\prfout^*_{i^*}$ uniformly at random, and thus the distribution of $\prfout^*$ does not change by this change.

\end{description}

$\hybi{5}$ is exactly the same as $\expb{\TPRF,\Sim,\qA}{sim}{cbp}(1^\secp,\coin=0)$.
This completes the proof of \cref{thm:TPRF-sim-cbp}.
\end{proof}




















%We define the algorithm $\qExtComp$ as follows.
%\begin{description}
%\item[$\qExtComp(\theta,(\SKE.\sk_i,\CPRF.\msk_i)_{i\in[n]},(\rho,\mat{U}))$:] $ $
%\begin{itemize}
%\item Inputs are $\theta\in\bit^n$, $n$ keys of $\SKE$ and $\CPRF$ $(\SKE.\sk_i,\CPRF.\msk_i)_{i\in[n]}$, and a quantum program with classical input and output $(\rho,\mat{U})$. Define a collection of binary outcome projective measurements $\cP$ in the same way as \cref{def:strong-PR-KLA}.
%\item Let $\{i_1,\ldots,i_\ell\}$ be the indices such that the corresponding bit of $\theta$ is $0$ (i.e., we have $\theta[i_j]=1$ for every $j\in[\ell]$.)
%\item Define the distribution $\tlD_j$ as follows for every $j\in[\ell]$.
%\begin{description}
%\item[$\tlD_j$:]Generate $\beta\gets\bit$, $\prfinp\gets\SKE.\Enc(\SKE.\sk_{i_j},\beta)$, $\cprfout_i\gets\CPRF.\Eval(\CPRF.\msk_i,\prfinp)$ for every $i\in[n]$. Set $\cprfout_0\seteq \bigoplus_{i\in[n]}\cprfout_i$ and sample $\prfout_1\gets\bit^\outlen$. Output $(\beta,\prfinp,\prfout_b)$.
%\end{description}
%\item Does the following from $j=1$ to $j=\ell$, where $\tlrho_1\seteq\rho$.
%\begin{itemize}
%\item Apply $\API_{\cP,\tlD_j}^{\epsilon,\delta}$ to $\tlrho_j$ and obtain the result $\tlp_j$ and the post state $\tlrho_j^\prime$.
%\item Set $x_{i_j}^\prime\seteq0$ if $\tlp_j>\frac{1}{2}$ and otherwise $x_{i_j}\seteq1$.
%\item Uncompute the previous steps and obtain a state $\tlrho_{j+1}$.
%\end{itemize}
%\item Output $(x_{i_j}^\prime)_{j\in[\ell]}$.
%\end{itemize}
%\end{description}
%
%\begin{proposition}
%Suppose we simulate $\hybi{1}$ to $\qA$ and obtain $\tlp>\frac{1}{2}+\gamma-\epsilon$.
%Then, if we execute $\qExtComp(\theta,(\SKE.\sk_i,\CPRF.\msk_i)_{i\in[n]},\allowbreak(\tlrho,\mat{U}))$, it holds that $x_{i_j}^\prime=x[i_j]$ with overwhelming probability for every $j\in[\ell]$, where $(x,\theta)$ and $(\SKE.\sk_i,\CPRF.\msk_i)_{i\in[n]}$ are used for the simulation of $\qA$, $(\rho,\mat{U})$ is the output of $\qA$, $\tlrho$ is the state after applying $\API_{\cP,D}^{\epsilon,\delta}$ to $\rho$, and $(x_{i_j}^\prime)_{j\in[\ell]}$ is the output of $\qExtComp$.
%\end{proposition}
%
%\begin{proof}
%a
%\end{proof}
%
%
%Using, $\qA$, we construct the following adversary $\qB=(\qB_0,\qB_1,\qB_2)$ that attacks the strong monogamy of entanglement property of BB84 states.
%\begin{description}
%\item[$\qB_0$:] Given an $n$-qubit BB84 states $\ket{\psi_1}\tensor\cdots\tensor\ket{\psi_n}$, $\qB_0$ first generates $\SKE.\sk_i\gets\bit^\secp$ and  $\CPRF.\msk_i\gets\CPRF.\Setup(1^\secp)$ for every $i\in[n]$ and generates $\CPRF.\sk_{i,b}\gets\CPRF.\Constrain(\CPRF.\msk_i,D[\SKE.\sk_i,b])$ for every $i\in[n]$ and $b\in\bit$.
%Let $U_i$ be the unitary that maps $\ket{u}\ket{v}$ to $\ket{u}\ket{v\oplus\CPRF.\sk_{i,u}}$.
%$\qB_0$ applies $U_i$ to $\ket{\psi_i}\ket{0\cdots0}$ and obtains $\qsk_i$ for every $i\in[n]$.
%$\qB_0$ then sends $(\qsk_i,\ldots,\qsk_n)$ to $\qA$.  When $\qA$ outputs a classical string $\cert$ and a quantum program with classical input and output $(\rho,\mat{U})$, $\qB_0$ sends $((\CPRF.\msk_{i})_{i\in[n]},(\rho,\mat{U}))$ to $\qB_1$ and $((\CPRF.\sk_{i,b})_{i\in[n],b\in\bit},\cert)$ to $\qB_2$.
%\item[$\qB_1$:] Given $\theta$ and $((\CPRF.\msk_{i})_{i\in[n]},(\rho,\mat{U}))$, $\qB_1$ first applies $\API_{\cP,D}^{\epsilon,\delta}$ to $\rho$ and obtains the result $\tlp$ and the post state $\tlrho_1$. If $\tlp\le\frac{1}{2}+\gamma-\epsilon$, $\qB_1$ outputs $\bot$. Otherwise, $\qB_1$ does the following. 
%\item[$\qB_2$:]Given $\theta$ and $((\CPRF.\sk_{i,b})_{i\in[n],b\in\bit},\cert)$, $\qB_2$ parses $\cert=(e_i,d_i)_{i\in[n]}$ and computes $x^\prime_i=e_i\oplus d_i\cdot(\CPRF.\sk_{i,0}\oplus\CPRF.\sk_{i,1})$ for every $i\in[n]$ such that $\theta[i]=1$.
%$\qB_2$ outputs $(x^\prime_i)_{i\in[n]:\theta[i]=1}$.
%\end{description}
%
%$\qB$ perfectly simulates $\hybi{3}$ for $\qA$.
%Let the BB84 state given to $\qB_0$ is generated from $x,\theta\in\bit^n$ and suppose $\qA$ wins in the simulated $\hybi{3}$. Then, we have
%\begin{align}
%e_i=x[i]\oplus d_i \cdot (\PKE.\dk_{i,0}\oplus\PKE.\dk_{i,1})
%\end{align}
%for $(e_i,d_i)$ for every $i\in[n]$ such that $\theta[i]=1$, from the condition that $\PKESKL.\Vrfy(\vk,\cert)=\top$.
%We also have
%\begin{align}
%m^\prime[i]=m^*[i]\oplus x[i]
%\end{align}
%for every $i\in[n]$ such that $\theta[i]=0$, from the winning condition on the final output $m^\prime$.
%From these facts, we have $\Pr[\hybi{3}=1]\le\Pr[\SMoEBB(\qB,n)=1]$.
%Thus, from the strong monogamy of entanglement property of BB84 states, we have $\Pr[\hybi{3}=1]=\negl(\secp)$.







==> omitted_proofs_lattice.tex <==
\section{Omitted Proofs in \Cref{sec:CS}}\label{sec:omitted_proofs_CS}
\input{proof_tail_bound}

\subsection{Proof of \Cref{lem:QSampGauss}}\label{sec:proof_QSampGauss}

\begin{proof}[Proof of \Cref{sec:proof_QSampGauss}.]
For all $q\ge 2$, we have\footnote{
$\sqrt{2\pi e}<5$ and $e^{\pi-\ln 2}>11$, and we have $5\sqrt{x}<11^x$ for all $x\ge 1$.}  
\[
\sqrt{\log q+1}\sqrt{2\pi e} \le e^{(\pi-\ln 2)(\log q+1)}.
\]
Thus, we have 
\[
6\left(\sqrt{\log q+1} \sqrt{2\pi e}\cdot e^{-\pi (\log q+1)}\right)^m
\le 
6(2q)^{-m}
=q^{-m}\cdot \negl(m).
\]
\end{proof}

==> preamble_newtheorem.tex <==
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}{Lemma} 
\newtheorem{claim}{Claim}  
\newtheorem{proposition}{Proposition} 
\newtheorem{definition}{Definition}  
\newtheorem{fact}{Fact}  
\newtheorem{remark}{Remark}  
%\newtheorem{proof}{Proof}  % Already defined by ``amsthm" package. Only include it when ``amsthm" is not used.
\newtheorem{corollary}{Corollary} 

==> preamble_usepackages_ex.tex <==

\usepackage[%
%  dvipdfmx, 
  colorlinks=true,
  citecolor=darkgreen,
  linkcolor=darkblue,
  urlcolor=darkblue,
  pagebackref=true
]{hyperref}

\usepackage{amsmath, amsfonts, amssymb, mathtools,amscd}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}



\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

\usepackage{etex}

\usepackage{arydshln} % In order to use \hdashline
\usepackage{url}
\usepackage{ifthen}
\usepackage{bm}
\usepackage{multirow}
\usepackage[dvips]{graphicx}
\usepackage[usenames]{color}
\usepackage{xcolor,colortbl} % Leave out in case the usepackage cannot be found. Not critical
\usepackage{threeparttable}
\usepackage{comment}
\usepackage{paralist,verbatim}
\usepackage{cases}
\usepackage{booktabs}
\usepackage{braket}
\usepackage{cancel} 
\usepackage{ascmac} 
\usepackage{framed}
% \usepackage{authblk}
\usepackage{pifont}
\usepackage{physics}
%\usepackage[dvipsnames]{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.6}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{maroon}{rgb}{0.5,0.1,0.1}
\definecolor{dpurple}{rgb}{0.2,0,0.65}
\definecolor{chocolate}{rgb}{0.8,0.4,0.1}

\usepackage[capitalise,noabbrev]{cleveref}
\usepackage[absolute]{textpos}
\usepackage[final]{microtype}
\usepackage[absolute]{textpos}
\usepackage{everypage}
\usepackage{autonum}

\usepackage{dsfont}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\ifnum\submission=1
\renewcommand*{\backref}[1]{}
\def\notxfont{1}
\pagestyle{plain}
\else
\fi


\ifnum\llncs=1
\renewcommand{\subparagraph}{\paragraph}
\else
\ifnum\notxfont=1
\else
\usepackage{mathpazo}
\usepackage{newtxtext}
\usepackage{helvet}
\fi
\fi


\newcommand{\heading}[1]{{\vspace{1ex}\noindent\sc{#1}}}

%%%%%%%%%%%%%%% Proof environment in non-LNCS style %%%%%%%%%%%%%%%%%%%
\newtheoremstyle{thicktheorem}%
{\topsep}
{\topsep}
{\itshape}{}%
{\bfseries}%
{.}
{ }%
{\thmname{#1}\thmnumber{ #2}%
		\thmnote{ (#3)}%
}

\newtheoremstyle{remark}%name
{\topsep}
{\topsep}
	{}%body font
	{}%indent amount
	{}%theorem head font
	{.}%punctuation after theorem head
	{ }%space after theorem head
	{\textit{\thmname{#1}}\thmnumber{ #2}%theorem head specs
			\thmnote{ (#3)}%
	}

\ifnum\llncs=0
	\theoremstyle{thicktheorem}
	\newtheorem{theorem}{Theorem}[section]
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{definition}[theorem]{Definition}

	\theoremstyle{remark}
	\newtheorem{claim}[theorem]{Claim}
	\newtheorem{remark}[theorem]{Remark}
	\newtheorem{example}[theorem]{Example}
	\newtheorem{note}[theorem]{Note}
	\newtheorem{conjecture}[theorem]{Conjecture}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


	\crefname{theorem}{Theorem}{Theorems}
	\crefname{assumption}{Assumption}{Assumptions}
	\crefname{construction}{Construction}{Constructions}
	\crefname{corollary}{Corollary}{Corollaries}
	\crefname{conjecture}{Conjecture}{Conjectures}
	\crefname{definition}{Definition}{Definitions}
	\crefname{exmaple}{Example}{Examples}
	\crefname{experiment}{Experiment}{Experiments}
	\crefname{counterexample}{Counterexample}{Counterexamples}
	\crefname{lemma}{Lemma}{Lemmata}
	\crefname{observation}{Observation}{Observations}
	\crefname{proposition}{Proposition}{Propositions}
	\crefname{remark}{Remark}{Remarks}
	\crefname{claim}{Claim}{Claims}
	\crefname{fact}{Fact}{Facts}
	\crefname{note}{Note}{Notes}

\ifnum\llncs=1
 \crefname{appendix}{App.}{Appendices}
 \crefname{section}{Sec.}{Sections}
\else
\fi

\ifnum\llncs=1
%\thispagestyle{empty}
\pagestyle{plain}
\renewcommand*{\backref}[1]{}
\else
	\renewcommand*{\backref}[1]{(Cited on page~#1.)}
	\ifnum\notxfont=1
	\else
		\usepackage{newtxtext}
	\fi
\fi


==> proof_tail_bound.tex <==
% !TEX root = main.tex
\subsection{Proof of \Cref{lem:strong_tail} }\label{sec:proof_strong_tail}
In this section, we prove \Cref{lem:strong_tail}. We prepare the following definitions and lemmata. 
\begin{lemma}[{\cite[Lemma 1.5]{Banaszczyk93}}]\label{lem:tail}
%For any lattice $\Lambda\subseteq \RR^m$,  $\sigma>0$, and $r\ge \frac{1}{2\pi}$,  
%\[
%\rho_\sigma(\Lambda\setminus  \mathcal{B}_m(r\sqrt{m}\sigma))\le \left(r \sqrt{2\pi e}\cdot e^{-\pi r^2}\right)^m\rho_{\sigma}(\Lambda)
%\]
%where $\mathcal{B}_m(r\sqrt{m}\sigma)=\{\vx\in \RR^m:\|\vx\|\le r\sqrt{m}\sigma\}$.  
For any $m$-dimensional lattice $\Lambda$, 
$\vt\in \RR^m$
$\sigma>0$, 
and $r\ge \frac{1}{2\pi}$,  
\[
\rho_\sigma((\Lambda+\vt)\setminus  \mathcal{B}_m(r\sqrt{m}\sigma))\le 2\left(r \sqrt{2\pi e}\cdot e^{-\pi r^2}\right)^m\rho_{\sigma}(\Lambda)
\]
where $\mathcal{B}_m(r\sqrt{m}\sigma)=\{\vx\in \RR^m:\|\vx\|\le r\sqrt{m}\sigma\}$. 
\end{lemma}
\begin{definition}
For any lattice $\Lambda$ and positive real $\epsilon>0$,  the smoothing parameter $\eta_\epsilon(\Lambda)$ is the smallest real $\sigma>0$ sucht hat $\rho_{1/\sigma}(\Lambda^*\setminus \{\vzero\})\le \epsilon$ 
where $\Lambda^*=\{\vx\in \RR^m: \forall \vz\in \Lambda, \langle \vx,\vz\rangle\in \ZZ\}$.
\end{definition}
\begin{definition}
For any lattice $\Lambda$, 
$\lambda_1^\infty(\Lambda):=\min_{\vx\in \Lambda\setminus \{\vzero\}}\|\vx\|_{\infty}$.
\end{definition} 
\begin{lemma}[{\cite[Lemma 2.7]{STOC:GenPeiVai08}}]\label{lem:shift_bound}
For any $m$-dimensional lattice $\Lambda$, $t\in \RR^m$, $\epsilon>0$, and $\sigma\ge \eta_\epsilon(\Lambda)$, 
\[
\rho_\sigma(\Lambda)\le \rho_\sigma(\Lambda+\vt)\frac{1+\epsilon}{1-\epsilon}.
\]
\end{lemma}

\if0
\begin{lemma}[{\cite[Combine Lemmas 2.6 and 5.3]{STOC:GenPeiVai08}}]
There is a constant $C>0$ such that the following holds. 
Let $n,m\in \NN$ and $q$ be a prime such that $m\ge 2n\log q$. 
For all but an at most $q^{-n}$-fraction of $\mA\in \ZZ_q^{n\times m}$, 
for any 
$\vy\in \ZZ_q^n$, 
\[
\eta_{1/2}(\Lambda_\mA^\vy)=C\sqrt{\log m}.
\]
%for a universal constant $C$. 
\end{lemma}
\fi



\begin{lemma}[{\cite[Lemma 2.6]{STOC:GenPeiVai08}}]\label{lem:smoothing_lower_bound}
    For any $m$-dimensional lattice $\Lambda$ and $\epsilon>0$, 
    \[
    \eta_\epsilon(\Lambda)\le \frac{\sqrt{\log(2m/(1+\epsilon^{-1}))/\pi}}{\lambda_1^\infty(\Lambda^*)}.
    \]
\end{lemma}

\begin{lemma}[{\cite[Lemma 5.3]{STOC:GenPeiVai08}}]\label{lem:lambda_1_lower}
Let $n,m\in \NN$ and $q$ be a prime such that $m\ge 2n\log q$. 
For all but an at most $q^{-n}$-fraction of $\mA\in \ZZ_q^{n\times m}$,  
\[
\lambda_1^\infty((\Lambda_\mA^\bot)^*)\ge 1/4. 
\]
%for a universal constant $C$. 
\end{lemma}

%The following lemma follows from \cite[Lemma 1.5]{Banaszczyk93} and\cite[Lemmas 2.6, 2.7, and 5.3]{STOC:GenPeiVai08}. See Appendix for the detail.
By combining the above lemmata, we prove \Cref{lem:strong_tail} as follows.
\begin{proof}[Proof of \Cref{lem:strong_tail}] 
By \Cref{lem:smoothing_lower_bound,lem:lambda_1_lower}, for all but an at most $q^{-n}$-fraction of $\mA\in \ZZ_q^{n\times m}$, 
\[
\eta_{1/2}(\Lambda)\le 4\sqrt{\log(2m/3)/\pi}.
\]
In particular, we can take a universal constant $C$ such that 
\[
\eta_{1/2}(\Lambda)\le C \sqrt{\log m}. 
\] 
For this $C$, if $\sigma\ge C \sqrt{\log m}$, then $\sigma\ge \eta_{1/2}(\Lambda)$, thus 
by \Cref{lem:tail,lem:shift_bound}, 
\begin{align}
 \frac{\rho_\sigma((\Lambda+\vt)\setminus  \mathcal{B}_m(r\sqrt{m}\sigma))}
 {\rho_{\sigma}(\Lambda+\vt)}\le 6\left(r \sqrt{2\pi e}\cdot e^{-\pi r^2}\right)^m.
    \end{align}
 By definition, 
\begin{align}
 \Pr_{\vx\gets D_{\Lambda_\mA^\vy,\sigma}}[\|\vx\|\ge r\sqrt{m}\sigma ]=
 \frac{\rho_\sigma((\Lambda+\vt)\setminus  \mathcal{B}_m(r\sqrt{m}\sigma))}
 {\rho_{\sigma}(\Lambda+\vt)}.
\end{align}
Thus, \Cref{lem:strong_tail} follows. 
\end{proof}

